Decompose-and-Compose: A Compositional Approach to Mitigating Spurious Correlation

While standard Empirical Risk Minimization (ERM) training is proven effective for image classification on in-distribution data, it fails to perform well on out-of-distribution samples. One of the main sources of distribution shift for image classification is the compositional nature of images. Specifically, in addition to the main object or component(s) determining the label, some other image components usually exist, which may lead to the shift of input distribution between train and test environments. More importantly, these components may have spurious correlations with the label. To address this issue, we propose Decompose-and-Compose (DaC), which improves robustness to correlation shift by a compositional approach based on combining elements of images. Based on our observations, models trained with ERM usually highly attend to either the causal components or the components having a high spurious correlation with the label (especially in datapoints on which models have a high confidence). In fact, according to the amount of spurious correlation and the easiness of classification based on the causal or non-causal components, the model usually attends to one of these more (on samples with high confidence). Following this, we first try to identify the causal components of images using class activation maps of models trained with ERM. Afterward, we intervene on images by combining them and retraining the model on the augmented data, including the counterfactual ones. Along with its high interpretability, this work proposes a group-balancing method by intervening on images without requiring group labels or information regarding the spurious features during training. The method has an overall better worst group accuracy compared to previous methods with the same amount of supervision on the group labels in correlation shift.

==> sec/4_related_work.tex <==
\section{Related Work}
\subsection{Mitigating Spurious Correlation}
It has long been known that deep models trained under standard ERM settings are vulnerable to spurious correlations\cite{bias, group, irm}. This problem has been addressed in the literature under terms such as shortcut learning\cite{shortcutlearning1, shortcutlearning2} and simplicity bias\cite{simplicitybias1, simplicitybias4}. 

\cite{LastLayer} states that models trained with ERM are capable of extracting both core and non-core features of an image and proposes to reweight the coefficients of features in the last layer of the predictor to make models robust to spurious correlations. Although this method has acceptable performance, it assumes that the group label of each validation data point is available, which is not feasible in many scenarios. Many methods have been proposed to retrain the last layer of models in the absence of group annotations \cite{AFR, disagreement}, most of which, are based on reweighting or selecting a subset of data for last layer retraining. As an example \cite{AFR} upweights samples for which a model trained with ERM assigns a low probability to the correct class. In addition to this line of work, \cite{jtt,LFF, diversify, Masktune, correctncontrast} introduce methods for fine-tuning whole models without group knowledge. \cite{jtt} upweights the data misclassified by a model trained by ERM to fine-tune a whole new model. \cite{diversify} trains two diverse classifiers and selects the one that performs better on the data from the minority group. \cite{Masktune}, which is the most similar work to ours, hypothesizes that models trained with ERM mostly focus on parts of the image with high spurious correlation to the label, and proposes to mask parts of the image with the highest scores according to xGradCAM. Then a new pretrained model is trained on the masked data.

\subsection{Using Synthetic Data for OOD Generalization}
tba.

\subsection{Attention-based Masking for Out-of-Distribution Generalization}
Some other works were proposed for removing the irrelevant parts of images by masking ~\cite{mask1, mask2}. \cite{caam} proposes a causal attention module that generates data partitions and removes confounders progressively to enhance models' generalizability. \cite{maskfinetune} masks patches of images based on the class activation map and refills them from patches of other images and utilizes these samples for distillation with a pretrained model. \cite{Masktune} masks the spurious parts of the image according to the class activation map and trains a new model on the masked data.
